RADICAL-Pilot and Parsl: Executing Heterogeneous Workflows on HPC Platforms

Workflows applications are becoming increasingly important to support scientific discovery. That is leading to a proliferation of workflow management systems and, thus, to a fragmented software ecosystem. Integration among existing workflow tools can improve development efficiency and, ultimately, increase the sustainability of scientific workflow software. We describe our experience with integrating RADICAL-Pilot (RP) and Parsl as a way to enable users to develop and execute workflow applications with heterogeneous tasks on heterogeneous high-performance computing resources. We describe our approach to the integration of the two systems and detail the development of RPEX, a Parsl executor which uses RP as its workload manager. We develop an RP executor that executes heterogeneous MPI Python functions on CPU cores and GPUs. We measure the weak and strong scaling of RPEX, RP, and Parsl when providing new capabilities to two paradigmatic use cases: Colmena and Ice Wedge Polygons

==> introduction.tex <==
%!TEX root = main.tex

The rapid development of compute-intensive data science applications defines new
opportunities for domain scientists to keep pace with the fast growth of the
technological progress on the one hand and introduces unexpected software and
application challenges on the other hand. Overcoming some of the software
challenges is approachable by developing new capabilities, yet other challenges
can be overtaken via interoperable, flexible, and reusable approaches. Among
examples of these software is RADICAL-Pilot (RP)~\cite{merzky2018using} workload
management and runtime system.

RP is designed to execute millions of
heterogeneous workloads on heterogeneous resources with no support for executing
workflows (API layer) and no support for executing Single Program Multiple Data
(SPMD) Message Passing Interface (MPI) functions (execution layer). RP is
designed to be a modular and portable system that enables a straightforward
integration approach with a 3rd party software without reengineering them.
Several 3rd party software such as Parsl-Pervasive Parallel Programming in
Python~\cite{babuji_2019_Parsl} and Flux~\cite{Dong_2014_Flux} offer the same
semantics and can be integrated on the scheduling or the execution level with
minimal effort.

Current computational and observational domain sciences use cases that deploy
different analysis algorithms are becoming more dependent on computations
involving many interrelated tasks. Further, as data-intensive scientific
workflows become the main driver for extreme-scale
science~\cite{Deelman2018future}, the use of parallelism, tailored workflow
management software, and High-Performance Computing (HPC) resources has become a
requisite requirement.

To address these challenges, we choose to integrate RP with Parsl for three
reasons: (i) RP and Parsl implementation is based on Python programming
language; (ii) Parsl provides an intuitive approach to expose parallelism via
simple and generic API; (iii) Parsl provides a simple approach to express data
flow dependencies with efficient workflow management capabilities. Similar to
RP, Parsl has no support to MPI SPMD
applications~\cite{Hadjidoukas_2020_torcpy}, we address this challenge by
implementing a single/multi-node non-MPI executor and single/multi-node MPI
function executor with direct support for the SPMD pattern.

We use two paradigmatic polar science use cases as an example of a larger domain
science class to characterize and analyze the performance of the integration on
SDSC Comet. The first use case consists of heterogeneous workflows that utilize
GPUs and CPUs to match large data set of satellite imagery. The second use case
consists of MPI workloads that use several GPUs and CPUs in an SPMD fashion to
process large satellite imagery of ~1.5 GB per image. We experimentally
characterize the performance of the stand alone non-MPI and MPI function
executors in terms of processing time and throughput on SDSC Comet and TACC
Frontera.

This paper offers four main contributions: (i) a complete description of the
architecture, design, and implementation of the RP-Parsl integration; (ii)
implementation of single/multi-node non-MPI and MPI function executor; (iii)
experimental characterization of the stand-alone executors on Comet and
Frontera; (iv) experimental characterization of the integrated system with two
exemplary Polar science use cases.

This paper's scope focuses on integrating two software systems, examining their
performance, and identifying the challenges of their integration. In addition,
this paper represents a preliminary examination of a broader approach to
developing a multi-level SDK from existing software. Exawork~\cite{exawork2021}
project represents the new approach of integrating a combination of
heterogeneous applications running on several heterogeneous compute nodes using
scalable workflow infrastructure to gear and manage the entire process.

We highlight and discuss the related works in~\S\ref{sec:related} and the
similar integration approaches between different systems, while distinguishing
RP-Parsl approach. We describe the implementation of the use cases and their
requirements in~\S\ref{sec:usecases}. In~\S\ref{sec:integration}, we show and
describe the integration of RP-Parsl in terms of design, architecture and
implementation.~\S\ref{sec:experiments} provides a performance characterization
of the stand-alone executors and the integrated system.
In~\S\ref{sec:conclusion}, we conclude the work of this paper and we illustrate
the future work.
